Bound-Based Power Optimization for Multi-Hop Heterogeneous Wireless Industrial Networks Under Statistical Delay Constraints

The noticeably increased deployment of wireless networks for battery-limited industrial applications in recent years highlights the need for tractable performance analysis methodologies as well as efficient QoS-aware transmit power management schemes. In this work, we seek to combine several important aspects of such networks, i.e., multi-hop connectivity, channel heterogeneity and the queuing effect, in order to address these needs. We design delay-bound-based algorithms for transmit power minimization and network lifetime maximization of multi-hop heterogeneous wireless networks using our previously developed stochastic network calculus approach for performance analysis of a cascade of buffered wireless fading channels. Our analysis shows an overall transmit power saving of up to 95% compared to a fixed power allocation scheme when using a service model in terms of the Shannon capacity limit. For a more realistic set-up, we evaluate the performance of the suggested algorithm in a WirelessHART network, which is a widely used communication standard for process automation and other industrial applications. We find that link heterogeneity can significantly reduce network lifetime when no efficient power management is applied. Moreover, we show, using extensive simulation study, that the proposed bound-based power allocation performs reasonably well compared to the real optimum, especially in the case of WirelessHART networks.

==> delay_bound_validation.tex <==
\subsection{Validation of the End-to-End Delay Bound}
\label{subsec:validation}
In this subsection we validate the end-to-end delay bound obtained from the kernel in Theorem~\ref{thm:1} using simulation.
%\subsubsection{Simulation Setup and Methodology}
%\label{subsubsec:sim_setup_shannon}
We simulate a multi-hop path consisting of Rayleigh-fading channels characterized by different mean channel gains $|{\bar{h}}_{n}^2|, \forall n$. 
Thus, the instantaneous SNR per hop $n$ in each time slot is exponentially distributed with mean $\gammabar_{n}$. %The transmission rate of each link is equivalent to the theoretical Shannon capacity.
We initially consider a transmission rate equal to the Shannon capacity, leading to a service characterization per time slot $i$ of link $n$ given by $s_{i,n}=\log g(\gamma_{i,n})= C \log_{2}(1+\gamma_{i,n})=\log(1+\gammabar_n h_{i,n}^2)^{\mathcal{C}}$, where again $\mathcal{C}=\nicefrac{C}{\log2}$. %where $B_s=N_s\log2$, $N_s$ is the number of payload symbols that can be transmitted per time slot and $|h_i|^2$ is the instantaneous channel gain. 
The Mellin transform for the cumulative SNR service process for link $n$ is then given by:  
\begin{equation}
\mathcal{M}_{\mathcal{S}}(s,\tau,t)=\left[e^{\nicefrac{1}{\gammabar_n}} \cdot {\gammabar_n}^{\mathcal{C}(s-1)} \Gamma\left(\mathcal{C}(s-1)+1,\nicefrac{1}{\gammabar_n}\right)\right]^{t-\tau}.
\end{equation}
%\begin{equation}
%\label{eq:service_shannon_mellin}
  %\mathcal{M}_{\mathcal{S}}(s,\tau,t)=\left[e^{\nicefrac{1}{\gammabar}} \cdot {\gammabar}^{\mathcal{C}(s-1)} \Gamma\left(\mathcal{C}(s-1)+1,\nicefrac{1}{\gammabar}\right)\right]^{t-\tau}.
%\end{equation}
For a constant arrival flow with data rate of $r_a$ bits per time slot, the respective cumulative arrival is defined as $A(\tau,t)=r_a(t-\tau)$ and its resulting Mellin transform in the SNR domain equals $\M_{\A}(s,\tau,t)=e^{ r_a (t-\tau)(s-1)}$. 
Then the kernel for the single hop system is obtained by substituting $\gammabar=\gammabar_n$ and $\M_{\alpha}\left(1 + s\right)=e^{r_a s}$ in Eq.~\eqref{eq:delay_kernel_rayleigh},
%\begin{equation}
%\label{eq:function_M}
  %\K(s,-\wepsilon)=\frac{\left(e^{\nicefrac{1}{\gammabar_n}} \cdot {\gammabar_n}^{-s\mathcal{C}}\cdot \Gamma(1-s\mathcal{C},\frac{1}{\gammabar_n})\right)^{w}}{1-e^{r_a s}\cdot e^{\nicefrac{1}{\gammabar_n}} \cdot {\gammabar_n}^{-s\mathcal{C}}\cdot \Gamma(1-s\mathcal{C},\frac{1}{\gammabar_n})} \leq \varepsilon\,,
%\end{equation}
for any $s>0$ for which the stability condition~\eqref{eq:stability_cond} holds. 
This kernel is subsequently used in order to obtain the end-to-end delay bound by applying Theorem~\ref{thm:1}.

For validation we use a fluid flow traffic model with constant rate $r_a$ and $C=20$ symbols per time slot.
We consider both 1-hop and 3-hop paths and compare the simulated delay violation probability to our analytical results ($\varepsilon$) for different delay bounds $w$.
We ran the simulation for $10^{8}$ time slots and collected samples from the end-to-end delay of the bits departing from the last link in order to empirically characterize the delay violation  probability for a given delay target.
All obtained statistics are presented with a 95\% confidence interval, but not always shown, due to their low absolute range. %In many cases in the following numerical results though the confidence levels were not printed due to their very low absolute range around the sample means of the violation probabilities.
%\subsubsection{Validation Results}
\begin{figure}
\centering
  \includegraphics[scale=0.42]{validation.pdf}
\caption{Comparison of the analytical upper bound of the delay violation probability with the simulated delay violation likelihood for 1-hop and 3-hop paths with the same bottleneck link with average SNR of 5 dB. The arrival rate is $r_a=20$ bits per time slot.}
\label{fig:2}
\end{figure}

A comparison of the analytical delay violation probability computed using Theorem~\ref{thm:1} with the empirical delay violation likelihood obtained via simulation versus the target delay is depicted in Fig.~\ref{fig:2}, which has also been presented in \cite{icc15}. Here we represent 1-hop and 3-hop paths, all having the same weakest link with average SNR of 5 dB. The figure reveals that the analytical bound is indeed an upper bound to the observed system performance. An important observation is that the decay rate for the computed delay violation probability is exactly the same as that obtained via simulation which suggests that the bound is asymptotically tight. Fig.~\ref{fig:2} further quantifies the effect of a bottleneck wireless link in a multi-hop path on the network performance and shows that it is affected by other links' qualities as well as the bottleneck link. Due to the big gap between the bottleneck link and the other links in the path with $\gammabar=\{15, 20, 5\}$ dB, this path yields almost the same performance as the 1-hop path, which is shown by both the simulation and analytical results. This observation suggests that managing the bottleneck link transmit power alone (or any other link in the path) may not result in the minimum power allocation for the desired delay performance.

The analytical and simulated delay violation probability versus the arrival rate are depicted in Fig.~\ref{fig:3}. We represent here different path lengths ($N=1$ and $N=3$) and two different target delays ($w=3$ and $w=5$ time slots). 
The average SNR is selected to be $\gammabar={5}$ dB in the 1-hop case and \mbox{$\gammabar=\{5,10,7\}$ dB} in the 3-hop case. 
%The figure reveals that the analytical bound is indeed an upper bound to the observed system performance.
Obviously, for both analytical and simulation results, the violation probability increases as the target delay becomes stricter. 
It also increases as the path length grows. 
The gap between the simulated and computed curves widens for larger arrival rates, which is expected due to the use of the union bound in the computation of the delay violation probability and since violation events become more probable at high system utilization. %implying in general that the analytical delay violation probability bound indeed is an upper bound to the empirical system behavior.
\begin{figure}
\centering
  \includegraphics[scale=0.24]{validation_arrival.png}
\caption{Comparison of the analytical upper bound of the delay violation probability with the simulated delay violation likelihood for a one-hop path with an average SNR of 5 dB and a 3-hop path with links $[5, 10 , 7]$ dB. The target delay is set to $w=\{3,5\}$ time slots.}
\label{fig:3}
\end{figure}


